Bicircular Light Induced Multi-State Geometric Current

We investigate the photocurrent induced by bicircular light (BCL) in materials, with a focus on its multi-state geometric nature. BCL, a combination of left- and right-circularly polarized light, can generate both injection and shift currents, originating from the geometric properties of gauge-invariant shift vectors, quantum geometric tensors, and triple-phase products. Crucially, the real parts of the quantum geometric tensors and triple-phase products remain nonzero in centrosymmetric systems, facilitating photocurrent generation in contrast to the traditional shift current bulk photovoltaic effect. Using a diagrammatic approach, we systematically analyze the BCL-induced photocurrents and demonstrate the multi-state geometric nature within a one-dimensional three-site Rice-Mele model. Our findings provide a quantum geometric understanding of BCL-induced photocurrents, underscoring the importance of considering multi-band contributions in real materials.

==> sections/feyn_diag/feyn_inj.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.6]{sections/feyn_diag/Feynman_inj.png}
    \caption{Third-order Feynman diagram depicting the injection current induced by BCL driving. The indices $\{\alpha, \beta, \gamma\}$ and $\{\mu\}$ represent the Cartesian coordinates of the three incident light beams and the output current respectively, while $\{a, b, c, d\}$ indicate the band indices of each Green's function.}
    \label{feyn diagram for injection current}
\end{figure}

==> sections/feyn_diag/feyn_sh.tex <==
\begin{figure}[ht]
    \centering  
    \includegraphics[scale=0.6]{sections/feyn_diag/Feynman_sh.png}
    \caption{Third-order Feynman diagram depicting the shift current induced by BCL driving. The indices $\{\alpha, \beta, \gamma\}$ and $\{\mu\}$ represent the Cartesian coordinates of the three incident light beams and the output current respectively, while $\{a, b, c, d\}$ indicate the band indices of each Green's function.}
    \label{feyn diagram for shift current}
\end{figure}

==> sections/section01_Geometry.tex <==
\section{Introduction} \label{sec:Introduction_geometry}
    The bulk photovoltaic effect (BPVE), a phenomenon where homogeneous materials generate a steady photocurrent under light illumination, has emerged as a cornerstone of modern optoelectronics\cite{BPVE_Wolfgang_1981, BPVE_Sipe_2000, BPVE_Fridkin_2001, BPVE_Andrew_2012, BPVE_Tan_2016, BPVE_Morimoto_2016}. Unlike conventional photovoltaic effects requiring interfaces (e.g., p-n junctions), BPVE driven by monichromatic light can arise intrinsically in noncentrosymmetric crystals\cite{BPVE_Fridkin_2001, BPVE_Andrew_2012}. This unique property enables novel applications in high-efficiency solar cells and polarization-sensitive photodetectors\cite{Application_BPVE_Grinberg_2013, Application_BPVE_Nie_2015}, driving extensive research over decades.
    \par
    A key challenge lies in activating BPVE in centrosymmetric materials, where inversion symmetry suppresses the effect. A promising strategy employs bicircular light (BCL)—a superposition of two counter-rotating circularly polarized beams with frequencies $n_1\omega$ and $n_2 \omega$\cite{BCL_Sipe_1996, BCL_Ikeda_Morimoto_2021, BCL_Habara_PRB_2023, BCL_Zhan_Blcak_Phosphorus_2024}. The resulting electric field forms a rose-like polarization pattern, dynamically breaking the material’s symmetry. The vector potential of BCL can be expressed as:
    \begin{equation}
        \begin{aligned}
            \boldsymbol{A}(t) = \boldsymbol{A}_R e^{in_1 \omega t} + \boldsymbol{A}_L e^{i(n_2 \omega t + \theta)} + \text{c.c.},
        \end{aligned}
    \end{equation}
    where $\boldsymbol{A}_{L/R}$ denotes the amplitude of the left- and right-circularly polarized light (LCP and RCP) and $\theta$ is the phase difference. $\theta$ controls the orientation of the polarization pattern. Notably, the $(n_1, n_2) = (1, 2)$ configuration induces a third-order nonlinear photocurrent in Dirac and Weyl semimetals\cite{BCL_Ikeda_Morimoto_2023, BCL_Kanega_graphene_2024}, with the phase $\theta$ serving as a knob to switch the current direction\cite{BCL_Ikeda_Morimoto_2024, BCL_Kanega_graphene_2024}. These advances highlight BCL’s potential for Floquet engineering and optoelectronic device design.
    \par
    The theoretical undertanding of BCL has been gradually built in recent years. It was first believed that injection currents that are proportional to relaxation time dominate the BCL-induced photocurrent\cite{BCL_tau1_Sipe_2000, BCL_tau1_Sipe_2012, BCL_tau1_Sipe_2014, BCL_Ikeda_Morimoto_2023}. In contrast, BCL can induce both injection and shift currents (the latter independent of relaxation time) in materials with centrosymmetry. A recent theoretical study by Ikeda et al. acknowledged this phenomenon and analyzed both injection and shift currents in Dirac electron systems\cite{BCL_Ikeda_Morimoto_2024}. They found that shift currents cannot be neglected and predicted the \(\theta\)-dependence for both types of light, a result that was later numerically validated by Kanega et al. in a tight-binding model of graphene by quantum master equation approach\cite{BCL_Kanega_graphene_2024}.
    However, the expression applicable to first principle calculation of BCL-induced photocurrent in real materials was still missing. Prior research also pointed out BCL-induced photocurrent may contain more than just pairwise-band contributions (involving two bands), but also multi-band contributions (involving more than two bands)\cite{BCL_Ikeda_Morimoto_2023}. But this effect has not been discussed in detail since it can be naturally neglected in a two-band model analysis. 
    \par
    Moreover, the constituent geometry quantities of BCL-induced photocurrent was still required further explanation. Nonlinear optics such as BPVE is a perfect platform to study geometric properties beyond traditional single-state level\cite{QGT_Provost_1980, QGT_PATI_1991, QGT_Cheng_2013}, since it naturally involves interband process. In previous researches, the geometry monochromatic light driven BPVE has been well-studied and proved to be strongly related to quantum geometric tensor and Levi-Civita connection\cite{Geometry_Ahn_PRX_2020,  Geometry_Ahn_NP_2022, Geometry_Avdoshkin_2023}. These geometric analyses provide a systematic understanding of the photocurrent and offer a framework for extending this knowledge to higher order nonlinear photocurrent.
    \par
    \input{sections/feyn_diag/Diagram_components}
    In our paper, we carried out a comprehensive analysis of BCL-induced photocurrent and answered the above questions. This paper is organized as follows. Section \ref{sec:Theoretical Background} presents a concise summary of the field theory formalism and the associated Feynman rules, building upon the foundational work of Parker and colleagues. Subsequent to this, Section \ref{BCL Induced Current} delineates the application of the diagrammatic approach to calculate the conductivities associated with the bicircular light (BCL)-induced current. Two resonant terms, injection and shift current, are studied in sequence, for their distinct relaxation time dependencies. A categorization of these conductivities is then performed by their containing composite geometry quantities. In addition to pairwise-band term, we identified multiband terms with both one singularity and double singularities. They are studied in detail from two aspects, featured geometry quantities and symmetry consideration. We then employs a three-band Rice-Mele Model in section \ref{sec:Model Example} to elucidate the physical mechanisms underlying BCL-induced photocurrent, with a particular emphasis on the multi-band contributions and the $\theta$-dependent photocurrent. Section \ref{sec:discussion} encapsulates the findings of the study in a concise manner. The Supplementary Material encompasses an in-depth analysis of the frequency integrals, a detailed exposition of the conductivities' calculations and their classification, as well as a symmetry analysis.

% Outline of Introduction
% short introduction to BPVE
% monochromatic light cannot induce photocurrent except for case P is broken
% short introduction to BCL
% short back of recent study On the one hand, expression for real material calculation is missing
% On the other hand, geometry is elusive. Previously, researches has bridge photocurrent and their corresponding geometry indication
% Outline of this paper


% Geometry -> relation between geometry and NLO
% Recently BCL has begun to draw attention due to its ability to induce photocurrent in P material. -> short introduction of BCL
% Shortcoming of recent study -> Geometry interpretation is unclear
%Floquet engineering is a potent technique for manipulating quantum systems using time-periodic external drives\cite{Floquet_review_Eckardt_2017, Floquet_review_Kitamura_2018, Floquet_Lindner_2011, Floquet_Rudner_2013, Floquet_Zhang_2016, Floquet_Rudner_2020, Floquet_Hu_2020, Floquet_Kitamura_2022}. Although this concept dates back several decades, it has gained renewed attention with advances in laser technology and ultrafast spectroscopy techniques\cite{Laser_Aoki_2014, Laser_Basov_2017}. The development of Floquet engineering has enabled a wide range of applications in diverse research fields, including ultracold atomic systems and optical lattices\cite{Floquet_application_Schuster_2021, Floquet_application_zhang_2023}. Moreover, with the growing industrial use of semiconductors, there is an increasing interest in nonlinear electronics\cite{Floquet_Semiconductor_SAWA_2008, Floquet_Semiconductor_Cario_2010, Floquet_Semiconductor_Oan_2014}, where Floquet engineering offers an effective approach for controlling semiconductor materials with exotic quantum properties.

%Moreover, the geometric interpretation of BCL-induced photocurrents remains unclear.  featured by different geometry quantities. We recovered the result that the pairwise-band contributions are characterized by the quantum geometric tensor as previous researches discussed\cite{QGT_Provost_1980, QGT_PATI_1991, QGT_Cheng_2013, QGT_Bernevig_2020, QGT_Wang_2022}. Meanwhile, the multi-band contributions are associated with another important geometric quantity—the triple phase product—which has been rarely studied in prior works \cite{Geometry_Triple_phase_product_Parks}.

% A common feature of geometric responses [1–15] is that they originate from inter-band hybridizations, such that they appear as quantum corrections to semiclassical descriptions. Since resonant optical responses are inherently inter-band quantum-mechanical processes, they are ideal candidates for a geometrical interpretation. Indeed, nonlinear optical responses, in particular, have attracted much attention recently for this reason [16–24] in addition to the possibility of diverse physical applications [25–27]. Quantized injection photocurrent responses were found in chiral semimetals [20–22], and the shift photovoltaic responses of semimetals have been found to be described by the Levi-Civita connection [19], a geometric quantity distinguished from the typical Berry curvature and quantum metric.

%The exploration of the geometry of quantum states in understanding the nonlinear and nonequilibrium responses of electronic systems to both static and dynamic electromagnetic fields has garnered significant attention, particularly evident in phenomena such as the nonlinear anomalous Hall effect[1] and shift current response[2-4]. Nonlinear optical responses transcend the realm of traditional single-state geometric properties, revealing as deeper connection to the underlying Riemannian geometry[5]. Notably, noncentrosymmetric materials exhibit even-order nonlinear photocurrent responses when subjected to an external electromagnetic field. A prominent example is the anomalous shift of charge carrier wave packets in real space through a second-order process upon photon excitation. This phenomenon, known as shift current, elucidates a mechanism crucial to understanding the bulk photovoltaic effect and is characterized by the shift vector, an interband geometrical property bridging two quantum states. Moreover, the shift vector plays a pivotal role in diverse phenomena like Landau-Zener tunneling[6], twisted Schwinger effect[7], high harmonic generation[8], and gauge invariant formulation of the semiconductor Bloch equations[9].  

%The understanding of relation between geometry of quantum states and non-linear optics has been gradually explored. Nonlinear optics naturally involves interband process.  

    %Among the various types of Floquet engineering, monochromatic circularly polarized light (CPL) is one of the most studied \cite{CPL_Nagaosa_2017, CPL_Watanabe_2021, CPL_Orenstein_2021, CPL_Dai_2023}. The properties and applications of CPL have been extensively explored, as it can induce a second-order injection current in non-centrosymmetric materials by breaking the internal time-reversal symmetry. 
    %\par
    %Recent years, bicircular light (BCL) began to draw increasing attention due to its characteristic ability to induce non-vanishing photocurrent in system with centrosymmetry. 
    %Nonlinear optics naturally involves interband process, requiring a generalization of traditional single-state geometric properties. In previous researches, understanding of relation between geometry of quantum states and non-linear optics has been gradually explored. Well-known examples are that second-order shift photocurrent and photovoltaic Hall effect has been explained to be associated to directly related to Levi-Civita connection and Hermitian curvature. These geometric analyses provide a systematic understanding of the photocurrent and offer a framework for extending this knowledge to other types of photocurrent.

    % replaced by deepseek
    %where $\boldsymbol{A}_{L/R}$ denotes the amplitude of the left- and right-circularly polarized light (LCP and RCP), and $\theta$ is the phase difference between them. The properties of BCL are strongly influenced by the input frequencies or the integer values $n_1$ and $n_2$, with different choices of these integers leading to distinct rose-like patterns, each breaking the intrinsic symmetry of the material. Among all BCL configurations, the pair $(n_1, n_2)$ = $(1, 2)$ is the most widely studied, as it induces a leading-order third-order photocurrent in centrosymmetric materials such as Dirac and Weyl semimetals\cite{BCL_Ikeda_Morimoto_2023, BCL_Ikeda_Morimoto_2024, BCL_Kanega_graphene_2024}. Furthermore, the phase difference $\theta$ plays a critical role in controlling the direction of the photocurrent, a fact highlighted in recent studies \cite{BCL_Ikeda_Morimoto_2024, BCL_Kanega_graphene_2024}. These characteristics of BCL significantly expand the potential applications of Floquet engineering and facilitate the artificial manipulation of photocurrent properties.


==> sections/table/classification_of_shift_current.tex <==
	\begin{table*}[ht]
			\centering
			\small

			\begin{tabular}{m{2cm}<{\centering} m{14cm}<{\centering}}
				\toprule
				\toprule
                \textbf{Composite Geometry} & \textbf{Expression} \\
                \midrule
                \midrule
                $ \partial R \times Q $ 
                &
				$
                \begin{aligned}
                    \frac{1}{3!}\frac{i\pi e^4}{2 \hbar^4 \Omega^3}\sum\limits_{\{\alpha, \beta, \gamma\}} \sum\limits_{ab} \int [d\boldsymbol{k}]f_{ab}h^{\alpha}_{ba}h^{\gamma}_{ab}\times \left[2\partial_{\mu}R^{\beta,\gamma}_{ab} \delta(\varepsilon_{ab} + \hbar\Omega) -  \partial_{\mu}R^{\beta,\alpha}_{ba} \delta(\varepsilon_{ab} + 2\hbar\Omega)\right]
                \end{aligned}
                $\\
				\midrule
				$ R \times R \times Q $
                &
				$
                \begin{aligned}
				\frac{1}{3!}\frac{\pi e^4}{2 \hbar^4 \Omega^3}\sum\limits_{\{\alpha, \beta, \gamma\}} \sum\limits_{ab} \int [d\boldsymbol{k}]f_{ab}h^{\alpha}_{ba}h^{\gamma}_{ab} \left(R^{\mu,\gamma}_{ab} - R^{\mu,\alpha}_{ba}\right)
				\left[ R^{\beta,\gamma}_{ab}2\delta(\varepsilon_{ab} + \hbar\Omega) + R^{\beta,\alpha}_{ba}\delta(\varepsilon_{ab} + 2\hbar\Omega) \right]    
                \end{aligned}
                $ \\
				\midrule
				$ \Delta \times R \times Q$
                &
				$
                \begin{aligned}    
                    &\frac{1}{3!}\frac{i\pi e^4}{2 \hbar^4 \Omega^3}\sum\limits_{\{\alpha, \beta, \gamma\}}\sum\limits_{ab} \int [d\boldsymbol{k}] f_{ab}\frac{h^{\alpha}_{ba}h^{\gamma}_{ab}}{\varepsilon_{ab}} \left\{\left[2\Delta^{\beta}_{ab}\left(R^{\mu, \gamma}_{ab} - R^{\mu, \alpha}_{ba}\right)\right]\left(5\delta(\varepsilon_{ab}+ \hbar\Omega) -2\delta(\varepsilon_{ab} + 2\hbar\Omega)\right)\right. \\
                    &\left.+\left[\Delta^{\mu}_{ab}\left(R^{\beta, \gamma}_{ab} - R^{\beta, \alpha}_{ba}\right)\right]\left(2\delta(\varepsilon_{ab}+ \hbar\Omega) +\delta(\varepsilon_{ab}+ 2\hbar\Omega)\right)\right\}
                \end{aligned}
                $ \\
				\midrule
				$ \Delta \times \Delta \times Q$
				&
				$
                \begin{aligned}
                    \frac{1}{3!}\frac{\pi e^4}{\hbar^4\Omega^3}\sum\limits_{\{\alpha, \beta, \gamma\}} \sum\limits_{ab} \int [d\boldsymbol{k}]f_{ab}\Delta^{\alpha}_{ab}\Delta^{\mu}_{ab}r^{\beta}_{ba}r^{\gamma}_{ab}\left[ 2\delta(\varepsilon_{ab} + \hbar\Omega) - \delta(\varepsilon_{ab} + 2\hbar\Omega)\right]]
                \end{aligned}
                $\\
				\midrule
				$ \Delta m \times Q$ 
                &
				$
                \begin{aligned}      
                    -\frac{1}{3!}\frac{\pi e^4}{2\hbar^4 \Omega^{3}}\sum\limits_{\{\alpha, \beta, \gamma\}} \sum\limits_{ab} \int [d\boldsymbol{k}]f_{ab}\Delta m ^{\mu\gamma}_{ab} \frac{h^{\alpha}_{ba}h^{\beta}_{ab}}{\varepsilon_{ab}}\left[5\delta(\varepsilon_{ab} + \hbar\Omega) +2 \delta(\varepsilon_{ab} + 2\hbar\Omega)\right] 
                \end{aligned}
                $\\
				\midrule	
				$R \times T \text{ [1S]}$
                &
				$
                \begin{aligned}
                    &\frac{1}{3!}\frac{i\pi e^4}{\hbar^4 \Omega^3}\sum\limits_{\{\alpha, \beta, \gamma\}}\sum\limits_{a\neq b\neq c} \int [d\boldsymbol{k}]\left\{\frac{1}{2}f_{ab}\left(\frac{1}{\varepsilon_{cb}} - \frac{1}{\varepsilon_{ac}}\right)\right.\\
				    &\times \left.\left[2T^{\alpha\beta\gamma}_{abc}\left(R^{\mu, \gamma}_{ac} + R^{\mu, \beta}_{cb} - R^{\mu, \alpha}_{ba}\right)\delta(\varepsilon_{ab} + \hbar\Omega) - \left(T^{\alpha\beta\gamma}_{abc}\right)^* \left(R^{\mu, \beta}_{bc} + R^{\mu, \gamma}_{ca} - R^{\mu, \alpha}_{ab}\right)\delta(\varepsilon_{ab} + 2\hbar\Omega)\right]\right\} \\
                    &+ \left\{ f_{ab} \times \left[T^{\alpha\beta\gamma}_{abc}\left(R^{\mu, \gamma}_{ac} + R^{\mu, \beta}_{cb} - R^{\mu, \alpha}_{ba}\right)\left(\mathcal{P}.\mathcal{V}. \frac{1}{\varepsilon_{ac} - \hbar\Omega} + \mathcal{P}.\mathcal{V}. \frac{1}{\varepsilon_{ac} + 2\hbar\Omega}\right)\delta(\varepsilon_{ab} + \hbar\Omega) \right. \right.\\
                    &\left.\left. - \left(R^{\mu, \gamma}_{ca} + R^{\mu, \beta}_{bc} - R^{\mu, \alpha}_{ab}\right)\left(T^{\alpha\beta\gamma}_{abc}\right)^*\mathcal{P}.\mathcal{V}. \frac{1}{\varepsilon_{ac} + \hbar\Omega}\delta(\varepsilon_{ab} + 2\hbar\Omega)\right]\right\}
                \end{aligned}
                $\\
				\midrule
				$\Delta \times T \text{ [1S]}$
                &
				$
                \begin{aligned}  
                    &-\frac{1}{3!}\frac{\pi e^4}{\hbar^4 \Omega^3}\sum\limits_{\{\alpha, \beta, \gamma\}}\sum\limits_{a\neq b\neq c} \int [d\boldsymbol{k}] \left\{\frac{1}{2}f_{ab}\left(\frac{1}{\varepsilon_{cb}} - \frac{1}{\varepsilon_{ac}}\right)\times\left(\frac{\Delta^{\mu}_{cb} - \Delta^{\mu}_{ac}}{\varepsilon_{cb} - \varepsilon_{ac}} - \frac{\Delta^{\mu}_{ba}}{\varepsilon_{ba}}\right) \right. \\
                    &\times \left. \left[2T^{\alpha\beta\gamma}_{abc} \delta(\varepsilon_{ab} + \hbar\Omega) - \left(T^{\alpha\beta\gamma}_{abc}\right)^* \delta(\varepsilon_{ab} + 2\hbar\Omega)\right]\right\}+ \left\{f_{ab}\left(\frac{\Delta^{\mu}_{ac}}{\varepsilon_{ac}}+ \frac{\Delta^{\mu}_{cb}}{\varepsilon_{cb}} - \frac{\Delta^{\mu}_{ba}}{\varepsilon_{ba}} \right) \right. \\
                    &\times \left. \left[T^{\alpha\beta\gamma}_{abc}\left(\mathcal{P}.\mathcal{V}. \frac{1}{\varepsilon_{ac} - \hbar\Omega} + \mathcal{P}.\mathcal{V}. \frac{1}{\varepsilon_{ac} + 2\hbar\Omega}\right)\delta(\varepsilon_{ab} + \hbar\Omega) - \left(T^{\alpha\beta\gamma}_{abc}\right)^*\mathcal{P}.\mathcal{V}. \frac{1}{\varepsilon_{ac} + \hbar\Omega}\delta(\varepsilon_{ab} + 2\hbar\Omega)\right]\right\}
                \end{aligned}
                $ \\
				\midrule
				$R \times T \text{ [2S]}$
                &
				$
                \begin{aligned}
				    &\frac{1}{3!}\frac{\pi^2 e^4}{\hbar^4 \Omega^3}\sum\limits_{\{\alpha, \beta, \gamma\}}\sum\limits_{a \neq b \neq c} \int [d\boldsymbol{k}]  f_{ab} T^{\alpha\beta\gamma}_{abc}
				    \\
				    &\left[f_{ab} \left(R^{\mu, \gamma}_{ac} - R^{\mu, \beta}_{cb}\right) + f_{bc} \left(R^{\mu, \alpha}_{ba} - R^{\mu, \gamma}_{ac}\right) + f_{ca} \left(R^{\mu, \alpha}_{cb} - R^{\mu, \gamma}_{ba}\right)\right]\delta(\varepsilon_{ab} + \hbar\Omega) \delta(\varepsilon_{bc} + \hbar\Omega)
                \end{aligned}
                $\\
				\midrule
				$\Delta \times T \text{ [2S]}$
                &
				$
                \begin{aligned}
				    &\frac{1}{3!}\frac{i\pi^2 e^4}{\hbar^4 \Omega^3}\sum\limits_{\{\alpha, \beta, \gamma\}}\sum\limits_{a \neq b \neq c} \int [d\boldsymbol{k}]  f_{ab}T^{\alpha\beta\gamma}_{abc}
				    \\
				    &\left[f_{ab} \left(\frac{\Delta^{\mu}_{ac}}{\varepsilon_{ac}} - \frac{\Delta^{\mu}_{cb}}{\varepsilon_{cb}}\right) + f_{bc} \left(\frac{\Delta^{\mu}_{ba}}{\varepsilon_{ba}} - \frac{\Delta^{\mu}_{ac}}{\varepsilon_{ac}}\right) + f_{ca} \left(\frac{\Delta^{\mu}_{cb}}{\varepsilon_{cb}} - \frac{\Delta^{\mu}_{ba}}{\varepsilon_{ba}}\right)\right]\delta(\varepsilon_{ab} + \hbar\Omega) \delta(\varepsilon_{bc} + \hbar\Omega)
                \end{aligned}
                $ \\
				\bottomrule
				\bottomrule
			\end{tabular}
			% \setlength{\abovecaptionskip}{0.4cm}
			\caption{Classification of conductivities for BCL-induced shift current based on their geometric and physical quantities. The shorthand notations used are as follows: $\varepsilon_{ab} = \varepsilon_a - \varepsilon_b$ represents energy differences; $\Delta^{\mu}_{ab} = \partial_{\mu}\varepsilon_{ab}$ denotes group velocity differences; $Q^{\alpha\beta}_{ab} = \frac{h^{\alpha}_{ba}h^{\beta}_{ab}}{\varepsilon^2_{ab}}$ is the quantum geometric tensor; $T^{\alpha\beta\gamma}_{abc} = h^{\alpha}_{ba}h^{\beta}_{cb}h^{\gamma}_{ac}$ represents the triple phase product; $\partial_{\mu}R^{\beta,\gamma}_{ab}$ is the shift vector dipole; $\Delta m^{\mu\alpha}_{ab} = \partial_{\mu}\partial_{\alpha}\varepsilon_{ab}$ is the inverse mass dipole. Products of these notations label the underlying quantities in each class, such as $\Delta \times R \times Q$, indicating terms with group velocity differences and the shift vector. The $[n\text{S}]$ notation highlights multi-band terms with $n$ singularities.}
			\label{shift currenty contribution}
		\end{table*}	

==> sections/table/symmetry_restriction_new.tex <==
%\begin{table}
%	\centering
%	\begin{tabular}{cc|cc|}
%		\hline
%		\multicolumn{4}{c}{\multirow{4}*{合并两行两列}}  & 三 & 四 \\
%		\cline{3-4}
%		\multicolumn{2}{c}{~} & 3 & 4 \\
%		\hline
%	\end{tabular}
%\end{table}

\begin{table}[ht]
    \renewcommand{\arraystretch}{1.3}
    \centering
    %\begin{tabular}{ccc|c}
    \begin{tabular}{m{1.5cm}<{\centering} m{3cm}<{\centering} m{2.5cm}<{\centering}}
        \hline
        \hline
		~ & \textbf{Singularity} &$\boldsymbol{\mathcal{T}}$\\
        \hline
        \multirow{2}*{\textbf{Injection}}& 1S & $\mathcal{I}$  \\
		~ & 2S & $\mathcal{R}$ \\
        \hline
        \multirow{2}*{\textbf{Shift}}& 1S & $\mathcal{R}$\\
        ~ & 2S & $\mathcal{I}$\\
        \hline
    \end{tabular}
    \setlength{\abovecaptionskip}{0.4cm}
    \caption{The non-vanishing part for each components of conductivity induced by BCL in material with time reversal symmetry $\mathcal{T}$, labeled by the surviving composite geometry quantities.}
    \label{surviving term in time reversal symetry}
\end{table}


% For convenience, we separate the geometry quantities we cared into real and imaginary part, and introduced several new shorthand notations. $\tilde{R}$ and $\tilde{I}$ are real and imaginary part of shift vector $R$, and they can be written as $\tilde{R}^{\alpha, \beta}_{ab} = \partial_{\alpha}\phi^{\beta}_{ab} + r^{\alpha}_{aa} - r^{\alpha}_{bb}$ and $\tilde{I}^{\alpha, \beta}_{ab} = i\partial_{\alpha}\ln\left(\abs{r^{\beta}_{ab}}\right)$, where we rewrite Berry connection as $r^{\beta} = \abs{r^{\beta}_{ab}} e^{-i\phi^{\beta}_{ab}}$. $g$ and $\Omega$ are both purely real and related to real and imaginary part of Quantum Geometry Tensor, where $Q^{\alpha\beta}_{ab} = g^{\alpha\beta}_{ab} - \frac{i}{2}\Omega^{\alpha\beta}_{ab}$. $\text{Re}T$ and $\text{Im} T$ are real and imaginary part of triple phase product.}
